Not Every Tree Is a Forest: Benchmarking Forest Types from Satellite Remote Sensing

Developing accurate and reliable models for forest types mapping is critical to support efforts for halting deforestation and for biodiversity conservation (such as European Union Deforestation Regulation (EUDR)). This work introduces ForTy, a benchmark for global-scale FORest TYpes mapping using multi-temporal satellite data1. The benchmark comprises 200,000 time series of image patches, each consisting of Sentinel-2, Sentinel-1, climate, and elevation data. Each time series captures variations at monthly or seasonal cadence. Per-pixel annotations, including forest types and other land use classes, support image segmentation tasks. Unlike most existing land use products that often categorize all forest areas into a single class, our benchmark differentiates between three forest types classes: natural forest, planted forest, and tree crops. By leveraging multiple public data sources, we achieve global coverage with this benchmark. We evaluate the forest types dataset using several baseline models, including convolution neural networks and transformer-based models. Additionally, we propose a novel transformer-based model specifically designed to handle multi-modal, multi-temporal satellite data for forest types mapping. Our experimental results demonstrate that the proposed model surpasses the baseline models in performance.

==> arxiv/sec/dataset.tex <==
\section{The \BenchmarkName\ dataset}

% \subsection{Reference data}

\begin{figure}[b]
	\centering
	\vspace{-1em}
    \includegraphics[width=0.8\linewidth]{sec/img/public_forty_200k_coverage_overall.png}
    % \includegraphics[width=0.5\textwidth]{sec/img/public_forty_200k_coverage_splits.png}
    \caption{\BenchmarkName\ dataset stratified random sample locations.}
    \label{fig:coverage}
\end{figure}

% data sources
To enable global wall-to-wall mapping, our reference data contain 8 classes: three forest classes (natural forest, planted forest, tree crops), other vegetation, water, ice, bare ground, and built areas. 
% natural
For \textit{natural} forest class, we integrate data from diverse sources to achieve a global coverage: primary humid tropical forests \citep{turubanova2018ongoing_primary2001}, primary forests in Europe \citep{sabatini2021european_euPrimary}, Canada \citep{maltman2023estimating_caPrimary}, and USA \citep{dellasala2022mature_usaPrimary}, natural forests from tropical moist forests (TMF) \citep{vancutsem2021long_TMF}, and natural lands from Science Based Targets Network (SBTN) \citep{Mazur_Sims_Goldman_Schneider_Pirri_Beatty_Stolle_Stevenson_SBTN}.
% planted
For \textit{planted} forest class, we merge planted forests from the planted areas from TMF \citep{vancutsem2021long_TMF} and SDPT \citep{richter2024SDPTv2}.
% tree crops
The \textit{tree crop} class integrates data from SDPT \citep{richter2024SDPTv2}, CORINE Land Cover \citep{cover2018copernicus_CORINE}, and tree crop species in cropland from national agricultural statistics service (USDA) \citep{nass2016usda} with several regional tree crop datasets covering a diverse range of tree crops, including palm, cocoa, rubber, coffee, coconut, cashew, and other orchards  \citep{kalischek2022_cocoaETH,  danylo2021_palmDanylo, vollrath2020angular_palmVollrath, descals2024global_palmDescals, fricker2022palmUcayali, souza2020mapbiomas, descals2023high_coconutDescals, sheil2024rubber, sourcecooperative2024_cashewBenin}.
% other vegetation
The \textit{other vegetation} class includes areas identified as shrubland, grassland, and cropland in WorldCover \citep{zanaga2021esa_worldcover2020} and areas labeled as vegetation in SBTN \citep{Mazur_Sims_Goldman_Schneider_Pirri_Beatty_Stolle_Stevenson_SBTN}. Only pixels confirmed by both data sources are assigned to the other vegetation class.
% other classes
For non-vegetation classes (\textit{water}, \textit{ice}, \textit{bare ground}, \textit{built areas}), we use labels from World Cover \citep{zanaga2021esa_worldcover2020}.

% \todo{Discuss "Unknown" class}
% In cases where a pixel cannot be unambiguously assigned to a single label, we assign the label \textit{unknown} and mask it out in the training.
% integrate all class layers
When integrating the three forest layers, we address disagreements between forest types by assigning a forest label only when there is consensus among the layers. In cases of disagreement, the pixels are labeled as \textit{unknown}. To incorporate non-forest classes, we use a tree height map \citep{potapov2022global_treemask}, adding non-forest labels only to areas where the tree height is less than 5~m. For regions affected by deforestation with high confidence of tree regrowth based on identified drivers \citep{sims2024drivers}, we assign planted forest label if no other valid label is applied.
% \todo{Discuss noise in the data: we do not expect 100\% accuracy of the labels, but rather want to encourage developing methods that are robust for a certain level of noise in the data.}
We acknowledge the presence of noise in these data sources. Our goal is to develop methods that can effectively handle such noise, reflecting the complexities of real-world scenarios.

\subsection{Satellite Data}
This benchmark dataset includes mutli-modal satellite inputs: Sentinel-2, Sentinel-1, climate, and elevation data (examples are shown in \autoref{fig:examples}).
\begin{itemize}
    \item \textbf{Sentinel-2} provides multispectral optical satellite imagery. For this benchmark, we extract seasonal and monthly mosaics from Sentinel-2 imagery for up to three years (2018-2020). We use 10 spectral bands with nominal resolutions of 10~m and 20~m, which are particularly useful for land cover mapping.
    \item \textbf{Sentinel-1} is a Synthetic Aperture Radar (SAR) satellite with 10~m resolution. Similar to Sentinel-2, we create mosaics for three years and use VV and VH polarizations from both ascending and descending orbits.
    \item \textbf{Climate} \citep{abatzoglou2018terraclimate} is a monthly climate dataset with a spatial resolution of approximately 4~km. This dataset provides key climate and water balance variables globally.
    \item \textbf{Elevation} is sourced from FABDEM \citep{hawker2022FABDEM}, based on Copernicus GLO 30 DEM with forests and buildings removed, providing elevation, slope, and aspect.
\end{itemize}


\begin{figure}
	\centering
    \includegraphics[width=\linewidth]{sec/img/examples/example_5cols_4.png}\\
    \includegraphics[width=\linewidth]{sec/img/examples/example_5cols_6.png}\\
    \includegraphics[width=\linewidth]{sec/img/examples/example_5cols_7.png}\\
    \includegraphics[width=\linewidth]{sec/img/colorbar_horizontal.png}\\
    \caption{Examples from left to right: (1) Sentinel-2 RGB bands, (2) Sentinel-2 SWIR-NIR-Red bands, (3) multi-temporal Sentinel-1 VV winter-spring-summer composition, (4) elevation, (5) labels. Bottom row: color bar for labels.\vspace{-0.9em}}
    \label{fig:examples}
\end{figure}


\subsection{Dataset Construction}

% sampling 
We use random stratified sampling to get locations distributed across the globe (see Figure~\ref{fig:coverage}), prioritizing forest type classes to ensure sufficient numbers of plots and pixels. The final dataset contains about 200,000 plots of 1280 $\times$ 1280 meter sizes. For each location, we extract satellite imagery and labels centered on the location.
%
To ensure geographically distinct datasets, we divide the world into $100\times 100\ km^2$ blocks and randomly assign them to the training, validation, and test sets in an 8:1:1 ratio. This approach guarantees that the training, validation, and test sets are geographically separated, reducing spatial autocorrelation and ensuring robust model evaluation.

\subsection{Dataset Analysis}
For the constructed benchmark, we compute the dominant class for each image sample. Approximately 13\% of the images are dominated by natural forest, 10\% by planted forests, 7\% by tree crops, and 17\% by other vegetation across the training, validation, and test sets. To further analyze the dataset, we investigate the class distribution based on the number of pixels and the number of distinct classes in each image, as illustrated in Figure~\ref{fig:class_distributions}.
%
% In the pixel distribution across classes, we observe that planted forests and tree crops occupy fewer pixels compared to natural forests and other vegetation. Despite efforts to encourage more balanced sampling during dataset construction, this imbalance is partly due to the nature of the data sources. For instance, tree crop data, such as the high-quality polygons in Brazil from \cite{coffeeCONAB}, are geographically concentrated, resulting in fewer total pixels. In contrast, data sources like \cite{turubanova2018ongoing_primary2001} for natural forests provide large-scale raster products that cover extensive areas.
%
In the pixel distribution across classes, we observe that planted forests and tree crops occupy fewer pixels compared to natural forests and other vegetation. While we use stratified sampling to prioritize forest type classes and achieve a more balanced distribution at the plot level, a perfectly balanced distribution at the pixel level is neither expected nor feasible. This imbalance reflects the diversity of the data and mirrors real-world conditions.
%
In the distribution of the number of classes per image, we find that most image samples contain at least four distinct classes. This indicates that by integrating diverse data sources, our benchmark provides rich segmentation labels, capturing the complexity and diversity of real-world land-cover scenarios.


\begin{figure}[hbt]
	\centering
	% Subfigure a: Number of pixels
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sec/img/histogram_pixel_distribution.png}
        \caption{Distribution of pixels across classes.}
        \label{fig:number_of_pixels}
    \end{subfigure}
    \hfill
    
    % Subfigure b: Number of classes
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{sec/img/histogram_numcls_image_distribution.png}
        \caption{Distribution of number of classes per image.}
        \label{fig:number_of_classes}
    \end{subfigure}
    
    % Main caption for the figure
    \caption{Overview of class distributions: (a) shows the distribution of pixels across classes, while (b) shows the distribution of the number of classes per image.\vspace{-0.9em}}
    \label{fig:class_distributions}
\end{figure}


==> arxiv/sec/intro.tex <==
\section{Introduction}

% importance
% Forests play a vital role in mitigating climate change by absorbing carbon dioxide from the atmosphere. Beyond their ecological significance, forests also provide invaluable social and cultural benefits. However, monitoring and managing these vital ecosystems presents significant challenges, particularly in the face of increasing deforestation rates.
% % a benchmark with detailed forest types is in need
% Existing forest maps and land use products often rely on a binary classification, distinguishing only between forested and non-forested areas \citep{turubanova2018ongoing_primary2001, sabatini2021european_euPrimary, zanaga2021esa_worldcover2020, brown2022_dynamicWorld}. While this approach provides a basic overview, it lacks the granularity needed to address complex challenges such as illegal logging and deforestation. With the implementation of regulations like the European Union Deforestation Regulation (EUDR), which requires tracking deforestation and degradation risk in supply chains, there is a growing need for more detailed forest typology maps. By differentiating between primary forests, planted forests, and tree crops, these maps can provide more accurate and informative data for policy-making, conservation efforts, and sustainable forest management \cite{richter2024SDPTv2}.
Forests play a crucial role in mitigating climate change while providing social, economic, and cultural benefits. It is especially important to differentiate between natural forests, planted forests, and tree crops to create actionable data supporting policy-making, conservation, and sustainable forest management \citep{richter2024SDPTv2}.
However, AI and computer vision research mostly focuses on forest recognition, differentiating only between forested and non-forested areas \citep{turubanova2018ongoing_primary2001, sabatini2021european_euPrimary, zanaga2021esa_worldcover2020, brown2022_dynamicWorld}. For instance, forest plantations for rubber or timber are still classified as forest cover\cite{zalles2024forestrethink}. While these maps provide a basic overview, they are inadequate for addressing deforestation risks and monitoring degradation, particularly under regulations like the European Union Deforestation Regulation (EUDR).

% The current definition of forests, such as that adopted by the Food and Agriculture Organization (FAO), defines a forest as land spanning more than 0.5 hectares with trees taller than 5 meters and a canopy cover exceeding 10\%. However, this definition prioritizes mapping forest extent over capturing deforestation dynamics and fails to distinguish between different forest types \citep{zalles2024forestrethink}. 
%
% As a result, forest maps typically rely on binary classifications, differentiating only between forested and non-forested areas \citep{turubanova2018ongoing_primary2001, sabatini2021european_euPrimary, zanaga2021esa_worldcover2020, brown2022_dynamicWorld}. For instance, the clearing of natural forests to establish plantations, such as rubber or timber, is still classified as forest cover. While these maps provide a basic overview, they are inadequate for addressing deforestation risks and monitoring degradation, particularly under regulations like the European Union Deforestation Regulation (EUDR). 
%


% DL
Satellite imagery and remote sensing, combined with machine learning, have become vital tools for forest monitoring. Foundation models trained on large-scale datasets are gaining traction in remote sensing but primarily capture general satellite image representations \citep{jakubik2023Prithvi, fuller2024croma}. A large-scale benchmark tailored for forest types mapping could advance this field and enable the development of forest-specific foundation models.
%
While existing forest-related machine learning benchmarks provide valuable resources, they have notable limitations. For instance, BigEarthNet \citep{sumbul2019bigearthnet} is a large dataset designed for deep learning but focuses on general land-cover classification rather than forest type mapping and provides only per-image labels. Regionally constrained datasets, such as TreeSatAI \citep{ahlswede2022treesatai} and BioMassters \citep{nascetti2024biomassters}, are tailored to specific forest-related tasks but are not designed for forest type mapping. A more closely related dataset is Planted \citep{pazos2024planted}, which utilizes the Spatial Database of Planted Trees (SDPT) \citep{richter2024SDPTv2} (a collection of data sources, including among others \citep{, Lesiv2022:gfm, roy2015:india, pan2011:noam-forests, furumo2017:oilpalm, petersen2016:tree-plantations}) to identify planted forests and tree crops. However, it also provides only per-image labels and lacks negative samples for non-planted forests. These limitations underscore the need for a comprehensive benchmark that enables detailed forest types mapping with per-pixel labels on a global scale.
% Satellite imagery and remote sensing, combined with machine learning techniques, have been widely used for forest monitoring. Recently, foundation models trained on large-scale datasets have gained traction in the remote sensing community, showing promise for general geospatial analysis. However, most existing foundation models, such as those based on self-supervised learning \citep{jakubik2023Prithvi,fuller2024croma}, are pretrained to capture general representation of satellite images. A large-scale deep learning benchmark specifically tailored for forest types mapping can not only foster forest types mapping but also enable the development of forest-specific foundation models.
% % limitations of current benchmarks
% Existing remote sensing benchmarks, including BigEarthNet \citep{sumbul2019bigearthnet}, Planted \cite{pazos2024planted}, Spatial Database of Planted Trees (SDPT) \cite{richter2024SDPTv2}, have contributed significantly to advancing machine learning for geospatial applications. However, they have several limitations. For instance, BigEarthNet \citep{sumbul2019bigearthnet} focuses on general land-cover classification and provides only per-image labels. Planted \citep{pazos2024planted} relies on the SDPT dataset to identify planted forests but provides per-image labels and lacks negative non-planted-forest samples. Other regional datasets like TreeSatAI \citep{ahlswede2022treesatai} and BioMassters \citep{nascetti2024biomassters} focus on a geographically limited region for a certain forest related task.

% characteristics and benefits of our benchmark
We introduce \BenchmarkName, a new global-scale, multi-modal multi-temporal benchmark  dataset designed to advance research in forest types mapping. \BenchmarkName\ features 200,000 globally distributed locations annotated with per-pixel labels and includes detailed forest classes: natural forests, planted forests, and tree crops, alongside non-forest categories. We propose a new transformer-based model (\MethodName) for forest type mapping and provide initial baselines results for the benchmark.


==> arxiv/sec/method.tex <==
% \section{Models}
\section{The \MethodName\ Model}

Attention mechanisms and transformers have become widely adopted in remote sensing applications \citep{garnot2021UTAE, tarasiou2023TSViT}. In this work, we benchmark against convolutional neural network (CNN) models, CNNs enhanced with attention mechanisms, and transformer architectures specifically designed for temporal satellite inputs. Building on Temporal-Spatial Vision Transformer (TSViT) \citep{tarasiou2023TSViT}, a ViT-based model tailored for time-series satellite data, we propose Multi-modal Temporal Spatial Vision Transformer (\textbf{\MethodName}) to handle multi-modal, multi-temporal inputs for per-pixel forest type mapping.

Figure~\ref{fig:model_overview} provides an overview of the model architecture. \MethodName\ consists of a spatial encoder, a temporal encoder, a multi-modal decoder, and a segmentation head to produce the per-pixel segmentation results. Both the encoders and the decoder are lightweight, consisting of two transformer layers, which effectively capture spatial, temporal, and multi-modal interactions.


% Image embedding
Following the standard transformer architecture for 3D patches, we patchify and project each satellite modality with the original shape $[B, T_m, H_m, W_m, C_m]$ into an embedding with the shape $[B, t_m, h_m, w_m, d]$. Here, $B$ denotes the batch size. $T_m$, $H_m$, $W_m$, and $C_m$ represent the original temporal, spatial, and channel dimensions of modality $m$, and $t_m$, $h_m$, $w_m$ are the patchified temporal and spatial dimensions of modality $m$. The embedding dimension, $d$, is set to 192.
% Spatial encoder
In both the spatial and temporal encoders, all modalities share the same encoders; thus, we omit the modality notation $m$ in the following description. The tensors are reshaped into $[Bt, hw, d]$ to focus the spatial encoder exclusively on processing tokens from the spatial dimension. For tensors from different modalities with varying $hw$, we pad them to the longest spatial dimension and mask irrelevant tokens in the attention layers. This enables the spatial encoder to handle modalities with differing spatial resolutions. Non-spatial satellite inputs, such as climate data, bypass the spatial encoder.
% Temporal encoder
After processing by the spatial encoder, the tensors are rearranged into $[Bhw, t, d]$, allowing the temporal encoder to focus solely on the temporal dimension. Additionally, we concatenate the sequence with $K$ class queries ($[Bhw, t+K, d]$), following the approach introduced in \cite{tarasiou2023TSViT}. We feed the resulted tensors into a standard transformer encoder. To eliminate the temporal dimension after the temporal encoder, we retain only the $K$ embeddings corresponding to the class queries ($[Bhw, K, d]$) and reshape them into $[BK, hw, d]$ for further processing.

% multi-modality decoder
In both the spatial and temporal encoders, we independently process image embeddings from each satellite modality. The multi-modality decoder is specifically designed to enable interaction among different modalities. This is achieved by using the embedding from one satellite modality as queries ($[BK, hw, d]$) and the embeddings from the other modalities as keys and values. For instance, climate and elevation features can be queried based on information from Sentinel-2 optical imagery. This approach leverages the standard transformer decoder to extract complementary features from other modalities guided by the context of a single modality. 
% segmentation head
Finally, a Multilayer Perceptron (MLP) is applied to project and reshape the decoder’s output into predictions, preserving the original spatial dimensions of the satellite modality used for querying.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{MTSViT_public_benchmark.pdf}
	\caption{An overview of the proposed model. The example demonstrates the use of two input modalities. The encoders are shared across modalities, while the decoder facilitates multi-modal interaction before the final segmentation head.\vspace{-0em}}\label{fig:model_overview}
\end{figure}


==> arxiv/sec/results.tex <==
\section{Experimental Results}

\subsection{Experimental Setup}

% introduce baselines
We evaluate our benchmark using three baseline models: \textbf{UNet3D}, a CNN-based model \citep{rustowicz2019:unet3d}, \textbf{UTAE}, a CNN model with temporal attentions \citep{garnot2021UTAE}, and \textbf{TSViT}, a transformer model specifically designed to process temporal satellite inputs \citep{tarasiou2023TSViT}.

% implementation details
For all baseline models and our proposed approach, we use the same implementation setup to ensure a fair comparison. Input channels are normalized using training set statistics. We train all models using the cross-entropy loss function. All implementations are developed in JAX \citep{jax2018github}. 
We train the models using a batch size of 64 for 40 epochs, with a learning rate of 0.001. We use the Adam optimizer with $\beta_1 = 0.9$, $\beta_2 = 0.9999$, and $\eta = 10^{-8}$.

% evaluation metrics
For the final evaluations, we train all models on the combined training and validation sets and evaluate them on the test set to report final performance metrics. To ensure robustness, we conduct repeated analyses with three different random seeds and report the average metrics. Per trained model, the performance is evaluated using the overall F1 score (macro-averaged across all classes) and the F1 score for forest classes (averaged over the three forest classes). Additionally, we report F1 scores for each forest type class.

\subsection{Main results}

We report the performance of baselines and our proposed \MethodName\ using seasonal Sentinel-2, climate, and elevation from 2020 as inputs, including standard deviations, in Table~\ref{tab:main_results}. Our model achieves the best performance across all metrics. The second-best performer is TSViT, which serves as the foundation for our proposed model. The key difference lies in the addition of a multi-modal decoder in \MethodName\ before the final segmentation head. This enhancement leads to a 1.8\% increase in forest F1 and 1\% to 2.7\% improvements for individual forest classes. CNN-based models, UNet3D and UTAE, show poorer performance, particularly for the planted forest and tree crop classes, which are more challenging due to their imbalanced distribution and smaller spatial coverage.

\begin{table}[hbt]
    \centering
    \caption{Results (F1 score and standard deviation) on the {\t test} set using Sentinel-2, climate, and elevation data over 1 year: \textit{Overall} F1, for the 3 \textit{Forests} classes, and for the individual forest types (natural (\textit{N}), planted (\textit{P}), and tree crops (\textit{TC})).
    }\label{tab:main_results}
    % \begin{tabular}{l|c|c|ccc}
    \begin{tabular}{lccccc}
    \toprule
           & \textbf{Overall} & \textbf{Forests} & \textbf{N} & \textbf{P} & \textbf{TC} \\ \midrule
    \textbf{UNet3D}   & 32.4 (1.3)    &24.2 (5.3)           & 56.2 (8.3)          &          7.5 (8.8) &    8.8 (12.1)      \\
    \textbf{UTAE}        &  49.4 (0.8)   & 37.7 (5.0)           &     71.4 (0.0)      &    13.8 (5.4)       &     27.8 (9.6)     \\
    \textbf{TSViT}       &   79.6 (0.1)  &    73.1 (0.1)        &     81.8 (0.0)      &    60.2 (0.3)       &   77.5 (0.2)       \\
    \textbf{Ours}     &  \textbf{81.1} (0.1)   &     \textbf{74.9} (0.1)       &      \textbf{82.8} (0.0)     &    \textbf{62.9} (0.3)       &  \textbf{78.9} (0.2)        \\ \bottomrule
    \end{tabular}
\end{table}

\subsection{Multi-modality ablation}

We evaluate the impact of different modality combinations on our proposed model using seasonal inputs from the year 2020. Figure~\ref{fig:multimodal} presents the performance across various input combinations. While the overall F1 score remains relatively consistent across inputs, we observe larger differences in the planted and tree crop classes. Incorporating elevation and climate data improves performance across all metrics, whereas the addition of Sentinel-1 shows minimal impact.

\begin{figure}[hbt]
	\centering
	\includegraphics[width=.8\linewidth]{sec/img/fig_multimodal_F1.png}
	\caption{Performance metrics across different satellite inputs combinations.}\label{fig:multimodal}
\end{figure}

\subsection{Multi-temporal ablation}

Our dataset includes monthly and seasonal satellite inputs spanning three years. We investigate how temporal resolution and the amount of data (in years) impact the results. Figure~\ref{fig:temporal} illustrates the performance of our model using Sentinel-2 data with varying temporal resolutions and years of input. The results clearly show that monthly and seasonal inputs significantly outperform annual inputs. While using more years of data further improves performance, the effect is less pronounced compared to the impact of temporal resolution.

\begin{figure}[hbt]
	\centering
	\includegraphics[width=.8\linewidth]{sec/img/fig_temporal_overallF1.png}
	\caption{Performance of overall F1 scores across different cadences (seasonal, monthly, and annual) over three years. The y-axis represents the F1 score as a percentage, while the x-axis indicates the number of years used.}\label{fig:temporal}
\end{figure}

==> not_used/sec/dataset.tex <==
\section{Dataset Description}

This section outlines the reference data sources and their integration into the final reference data. It then details the satellite data used as input and the process of assembling the deep learning (DL) dataset through balanced sampling, considering geographic locations and class frequency. Finally, the section introduces the various variants of the dataset.


\subsection{Reference data}

\subsubsection{Natural and planted forest}

For natural forest, the reference data is a combination of Primary Humid Tropical Forests (Primary) \cite{turubanova2018ongoing_primary2001}, Spatial Database of Planted Trees (SDPT) \cite{richter2024SDPTv2}: use planted and tree crops polygons, Primary forests in Europe (EU Primary) \cite{sabatini2021european_euPrimary}, 

\begin{itemize}
    \item Primary Humid Tropical Forests (Primary) \cite{turubanova2018ongoing_primary2001}
    \item Spatial Database of Planted Trees (SDPT) \cite{richter2024SDPTv2}: use planted and tree crops polygons
    \item Primary forests in Europe (EU Primary) \cite{sabatini2021european_euPrimary}: natural forest
    \item Primary forests in Canada (CA Primary) \cite{maltman2023estimating_caPrimary}: natural forest
    \item Primary forests in USA (USA Primary) \cite{dellasala2022mature_usaPrimary}: consist of forest layers generated for different years, mapped to natural forest
    \item Tropical moist forests (TMF) \cite{vancutsem2021long_TMF}: natural, secondary, planted forest
    \item Natural lands from Science Based Targets Network (SBTN) \cite{Mazur_Sims_Goldman_Schneider_Pirri_Beatty_Stolle_Stevenson_SBTN}: ???
    \item Forest height map from Global Land Cover and Land Use change (GLCLU) 2020 \cite{potapov2022global_treemask}: we use forest height map from GLCLU in 2020 as a tree mask (select trees at least 5~m high)
    \item Forest loss from \cite{hansen2013high_Hansen_forestloss}: we use forest loss year to find lands suffered from deforestation during 2000 to 2020.
    \item Drivers \todo{citation of drivers work}
\end{itemize}

Natural forests: combine Primary, EU Primary, CA Primary, USA Primary, TMF natural, TMF secondary, SBTN natural.
Planted forests: combine planted forests from SDPT and TMF planted.

\subsubsection{Tree crops}
\begin{itemize}
    \item Coffee CONAB \cite{coffeeCONAB}
    \item Palm Danylo \cite{danylo2021_palmDanylo}, Palm Vollrath \cite{vollrath2020angular_palmVollrath}, Palm Descals \cite{descals2024global_palmDescals}, Palm Ucayali \cite{fricker2022palmUcayali}
    \item Cocoa ETH \cite{kalischek2022_cocoaETH}
    \item Rubber Sheil \cite{sheil2024rubber}
    \item Coconut Descals \cite{descals2023high_coconutDescals}
    \item Cashew Benin \cite{sourcecooperative2024_cashewBenin}
    \item CORINE 2012 \cite{cover2018copernicus_CORINE}: fruit trees and olive groves, and agro-forestry areas
    \item USDA 2020 \cite{nass2016usda}: select tree crops species from cropland
\end{itemize}

Tree crops: combine those tree crops sources with tree crops from SDPT.

\subsubsection{Other non-forest classes}
\begin{itemize}
    \item World Cover \cite{zanaga2021esa_worldcover2020}: water, ice, bare ground, built areas, other vegetation (shrubland, grassland, cropland).
\end{itemize}
We use tree mask to double check those non-forest classes.


\subsubsection{Further data processing for forest classes}
% how to handle tree disagreement.
When combining the three forest classes, we prioritize tree crops over planted forests and natural forests. If multiple sources label the same pixel with different forest types, we assign the pixel to the highest-priority class. For instance, if both natural forests and tree crops sources label a pixel, we classify it as a tree crop.

% 5 exp flags in pp_ops.
% strcit_veg
For other vegetation, we combine labels from World Cover and SBTN, and then refine the results using a tree mask to exclude areas with trees taller than 5 meters.
% drop_veg_after_deforestation
As it is hard to examine what happens to the land after a deforestation event, we utilize forest loss labels from \cite{hansen2013high_Hansen_forestloss} to find lands suffered from deforestation during 2000 to 2020. These areas are classified as other vegetation instead of any forest types.
% use_weak_tree_crops / use_weak_planted
We check the disagreement between three forest types. We only assign tree crops or planted forest labels when there is no disagreement.
% use_drivers
For areas affected by deforestation where there is high confidence of tree regrowth based on identified drivers \todo{citation of drivers work}, we assign a ``planted forest" label if no other valid label is available.

\begin{table*}[]
\caption{A summary of reference data sources}
\label{tab:data_source_summary}
\begin{tabular}{llllll}
\hline
\textbf{Data source} & \textbf{Classes} & \textbf{Resolution} & \textbf{Year} & \textbf{Region} & \textbf{Count} \\ \hline
         Primary \cite{turubanova2018ongoing_primary2001}            &       forest           &        30~m             &     2001          &      tropics           &      raster from Landsat          \\
         SDPT  \cite{richter2024SDPTv2}          &      natural,planted,tree crops            &       10~m              &    mainly 2020           &     global            &   2M polygons             \\ 
         World Cover \cite{zanaga2021esa_worldcover2020}           &     others             &         10~m            &     2020          &       global          &     raster from S1 \& S2          \\ 
        EU Primary  \cite{sabatini2021european_euPrimary}           &      natural            &        -             &     2000-2019          &    Europe             &                points \& polygons integrated \\
        CA Primary  \cite{maltman2023estimating_caPrimary}           &       forest           &        30~m             &      2019         &     Canada            &   raster from Landsat             \\ 
        USA Primary  \cite{dellasala2022mature_usaPrimary}           &       forest           &       30~m              &      -         &     USA            &    raster from Landsat            \\ 
        TMF \cite{vancutsem2021long_TMF}             &      natural,planted            &      30~m               &    1990-2019            &   tropics             &   raster from Landsat             \\ 
        SBTN  \cite{Mazur_Sims_Goldman_Schneider_Pirri_Beatty_Stolle_Stevenson_SBTN}           &    natural              &             30~m        &     2020    & global       &   raster based on other layers from Landsat \& SDPT             \\ 
        GLCLU \cite{potapov2022global_treemask}             &         forest         &      30~m               &      2020         &      global           &       raster from Landsat         \\
        Forest loss \cite{hansen2013high_Hansen_forestloss}             &     forest             &         30~m            &    2000-2022           &  global              &  raster from Landsat              \\ 
        Drivers \todo{citation of drivers work}              &    forest              &                     &               &                 &                \\ 
        Coffee CONAB \cite{coffeeCONAB}            &   tree crops               &      -               &     2016-2019          &    Brazil             &  411k polygons              \\ 
        Palm Danylo \cite{danylo2021_palmDanylo}            &      tree crops            &       -              &    2017           &   SE Asia              &       5k points         \\ 
        Palm Vollrath  \cite{vollrath2020angular_palmVollrath}           &tree crops & -                    &   2017            &     Tropics            &     5145 points           \\ 
        Palm Descals  \cite{descals2024global_palmDescals}           &       tree crops           &        -             &     2016-2021          &    tropics             &    17812 points            \\ 
        Palm Ucayali \cite{fricker2022palmUcayali}             &        tree crops          &         -            &   2020            &    Peru             &      1.2k polygons          \\ 
        Cocoa ETH   \cite{kalischek2022_cocoaETH}          &      tree crops            &     10~m                &   2018-2021            &      Côte d'Ivoire \& Ghana           &     raster from Sentinel-2           \\ 
        Rubber Sheil \cite{sheil2024rubber}            &      tree crops            &       -              &     \todo{paper is not accessible} ??         &   SE Asia              &      1.5k points          \\ 
        Coconut Descals  \cite{descals2023high_coconutDescals}           &       tree crops           &        -             &      2020         &   SE Asia, India              &   300 points             \\ 
        Cashew Benin   \cite{sourcecooperative2024_cashewBenin}          &      tree crops            &     50~cm                &    2020           &      Benin, West Africa           &    annotated based on Airbus Pleiades images            \\ 
        CORINE   \cite{cover2018copernicus_CORINE}         &      tree crops            &    100~m                 &     2012          &   Europe              &      raster  from S2 \& S1        \\ 
        USDA    \cite{nass2016usda}         &     tree crops             &      30~m               &    2020           &     USA            &      raster from Landsat          \\ 
                     &                  &                     &               &                 &                \\ 
                     

\hline
\end{tabular}
\end{table*}

\subsection{Input data}
\begin{itemize}
    \item Sentinel-2
    \item Climate
    \item Elevation
\end{itemize}

\subsection{Dataset Assembly}
% geographic sampling & balanced sampling

% talk about different versions of dataset

\begin{itemize}
    \item 50k-non-Temporal
    \item 50k
    \item 200k-non-Temporal
    \item 200k
\end{itemize}

\subsection{Benchmark statistics}

\todo{a figure of dataset coverage and train/test split}

\todo{histogram of class frequency}

==> not_used/sec/discussion.tex <==
\section{Discussion and Conclusion}

==> not_used/sec/experiment.tex <==
\section{Experiments}

\subsection{Experiment setup}

Baselines.
We benchmark our approach against 4 recent state-of-the-art methods: \todo{need to rewrite baselines, currently copied from SoAm draft}
\begin{itemize}
    \item \textbf{UNet3D}: UNet model with 3D convolutions \todo{check the reference paper inside google codes}. For multi-modality inputs, we resize all modalities into the same shape and concatenate them along channel dimension.
    \item \textbf{U-Net with Temporal Attention Encoder (UTAE)}: a model based on the UNet architecture incorporating an attention layer to address the temporal dimension. \cite{garnot2021UTAE}. We adopt the late fusion technique introduced in \cite{garnot2022PASTIS-R} to manage multi-modality inputs. Inputs are resized to the same spatial dimensions to facilitate feature concatenation during late fusion.
    \item \textbf{Temporal-Spatial Vision Transformer (TSViT)}: a transformer-based model with separate modules to handle spatial and temporal dimensions \cite{tarasiou2023TSViT}. Similar to UNet3D, TSViT is not originally designed for multi-modality inputs. Therefore, we resize all inputs to the same shape and concatenate them.
\end{itemize}

Metrics.
\begin{itemize}
    \item overall F1
    \item F1, Precision, Recall of each forest type class
\end{itemize}

\subsection{Implementation details}

\subsection{Experiment results}

\todo{a figure of predictions from different models}

\paragraph{Model comparison}


\paragraph{Multi-modality input}


\paragraph{Temporal analysis}


\subsection{Model ablation}

\begin{itemize}
    \item Separate spatial encoders
    \item With and without multi-scale decoder
\end{itemize}

==> not_used/sec/intro.tex <==
\section{Introduction}

%%% intro-intro %%% 
% forest typology mapping is important 
Forests play a vital role in mitigating climate change by absorbing carbon dioxide from the atmosphere. Beyond their ecological significance, forests also provide invaluable social and cultural benefits. However, monitoring and managing these vital ecosystems presents significant challenges, particularly in the face of increasing deforestation rates.
% a benchmark with detailed forest types is in need
Existing forest maps often rely on a binary classification, distinguishing only between forested and non-forested areas. While this approach provides a basic overview, it lacks the granularity needed to address complex challenges such as illegal logging and deforestation. With the implementation of regulations like the European Union Deforestation Regulation (EUDR), which requires tracking deforestation and degradation risk in supply chains, there is a growing need for more detailed forest typology maps. By differentiating between primary forests, planted forests, and tree crops, these maps can provide more accurate and informative data for policy-making, conservation efforts, and sustainable forest management \cite{richter2024SDPTv2}. \todo{a teaser figure: visualize a patch of world cover, our label, our prediction}
% satellite data and DL
Satellite imagery and remote sensing, combined with machine learning techniques, have emerged as powerful tools for forest monitoring. Publicly accessible satellite data enable large-scale forest mapping, and machine learning models effectively capture intricate feature patterns, yielding impressive results. However, two key challenges persist. Firstly, raw satellite data is often voluminous and requires significant processing to prepare it for machine learning applications. Secondly, most machine learning methods rely on supervised learning, demanding substantial amounts of reference data. To foster further research and development in forest mapping, particularly leveraging recent advancements in deep learning, there is a pressing need for a readily accessible benchmark dataset specifically tailored for forest typology mapping. This benchmark should encompass both processed satellite data and accurate reference labels.
% our work
Therefore, we introduce a new global-scale, multi-temporal benchmark for forest typology mapping, focusing on these three key forest classes, primary forest, planted forest, and tree crops.
% We frame this benchmark as an image segmentation task for deep learning-based supervised learning. By evaluating deep learning baselines on this benchmark and leveraging the recent advancements in deep learning, we aim to stimulate further research and advancements in forest typology mapping.

%%% problem %%% 
% what are the current related works, what are their limitations.
% only one class: forest maps and land use products.
Existing studies on forest typology mapping often focus on a single, general forest class. For instance, the primary humid tropical forest map from \cite{turubanova2018ongoing_primary2001} provides a 30-meter resolution map for forest monitoring in the tropics in 2001. While valuable for forest monitoring, this binary product offers only one forest class. Similarly, other forest maps, such as those by \cite{sabatini2021european_euPrimary}, \cite{dellasala2022mature_usaPrimary}, and \cite{maltman2023estimating_caPrimary}, and land use products like World Cover (\cite{zanaga2021esa_worldcover2020}) and Dynamic World (\cite{brown2022_dynamicWorld}), also provide a single forest class.
% planted forest.
Recently, there has been growing interest in more detailed forest typology information. \cite{vancutsem2021long_TMF} provide a map distinguishing natural and planted forests in the tropics. \cite{richter2024SDPTv2} offer worldwide polygons for planted and tree-crop classes. 
% tree crops. more challenging.
Tree crops, particularly, present a more challenging class to map compared to natural and planted forests. While existing global-scale land use products like World Cover and Dynamic World include crop and tree classes, they do not differentiate between tree crops and other types of trees. Regional maps, such as the Copernicus Land Cover Map (\cite{cover2018copernicus_CORINE}) for Europe and the USDA National Agricultural Statistics Service (NASS) data for the USA, provide tree crop classes like fruit trees and olive groves at 100-meter and 30-meter resolutions, respectively. Additionally, numerous localized, single-species tree crop datasets are available. For example, studies by \cite{danylo2021_palmDanylo}, \cite{descals2024global_palmDescals}, and \cite{vollrath2020angular_palmVollrath} provide 5,000 to 10,000 palm points in the tropics. Similar localized datasets exist for other tree crops, including cocoa (\cite{kalischek2022_cocoaETH}), coconut (\cite{descals2023high_coconutDescals}), and cashew (\cite{sourcecooperative2024_cashewBenin}). By combining these tree crop data sources with existing maps of natural and planted forests, a robust dataset for forest typology mapping can be created.

% the trend of using DL-methods for forest typology mapping, so need a benchmark tailored for it
\todo{some works of DL in forest mapping, vegetation paramter estiamtino, etc.}


%%% state our research objective %%% 
% so what are the required characteristics of a good benchmark for forest typology mapping 
% detailed forest types, global-scale, multi-temporal, ready for DL-based supervised learning
We aim to create a benchmark for forest typology mapping, distinguishing between three key forest classes: natural forests, planted forests, and tree crops. This benchmark is designed to streamline deep learning model training and testing by providing well-formatted input and reference data. This approach saves researchers time and encourages more extensive exploration of forest-related models.
%
As a large-scale, globally-comprehensive benchmark, it is suitable for training generalist models for diverse forest applications. Additionally, it can serve as a testbed for remote sensing foundation models trained using self-supervised learning. To capture seasonal variations, particularly in tree crops, we provide multi-temporal input data to facilitate the exploration of temporal dimensions in model development.


The main contributions of this paper include:
\begin{itemize}
    \item We introduce a novel global-scale, multi-temporal benchmark for forest typology mapping. This benchmark, constructed from a diverse range of satellite imagery and reference labels obtained from multiple public data sources, provides a valuable resource for the remote sensing community.
    \item We conduct an evaluation of learning methods on the proposed benchmark, shedding light on their strengths and limitations in the context of forest typology mapping.
    \item By making this benchmark publicly accessible, we aim to accelerate advancements in deep learning techniques for forest typology mapping, ultimately contributing to improved forest monitoring and management practices.
\end{itemize}

==> not_used/sec/method.tex <==
\section{Methodology}

\subsection{The proposed model \MethodName} \todo{need to rewrite baselines, currently copied from SoAm draft}
We work with a dataset denoted as $\mathcal{D}=\{(X_n, Y_n), n \in [\![ 1, N ]\!] \}$, comprising $N$ samples, where $X_n$ represents the input tensors and $Y_n$ denotes the reference data. Each $X_n$ comprises time series images collected from $M$ different satellites, thus forming a dictionary structure where each element $X_n^m$ corresponds to data from a specific satellite. Notably, each $X_n^m$ has dimensions $[T_m, H_m, W_m, C_m]$, representing the temporal ($T_m$), spatial ($H_m, W_m$), and channel ($C_m$) dimensions, which may vary across the $M$ satellites. The reference, $Y_n$, has the shape of $[H, W, K]$, where $H, W$ are the same as the spatial dimensions of one chosen modality in $X_n$ and $K$ is the number of segmentation classes.

% \begin{figure}[th]
%   \centering
%   \includegraphics[width=.95\textwidth]{img/mtsvit.drawio.png}
%   \caption{\textbf{Overview of the proposed method.} $X$ refers to the batched input tensors containing multiple modalities and $y_{pred}$ is the segmentation prediction.
%   }
%   \label{model_overview}
% \end{figure}

Figure \ref{model_overview} illustrates the model architecture overview. The proposed model comprises a spatial encoder, a temporal encoder, and a multi-modality decoder. As the normal transformer architecture used in segmentation task, we patchify images at the beginning and use a segmentation head in the end.

\paragraph{Image embedding}
For each satellite, we patchify and transform its batched input tensors from dimensions $[B, T_m, H_m, W_m, C_m]$ into dimensions $[B, t_m, h_m, w_m, c_m]$, where $B$ represents the batch dimension, and $c_m$ is calculated as $p_m^t \times p_m^h \times p_m^w \times C_m$. Here, $[p_m^t, p_m^h, p_m^w]$ denotes the patch sizes specific to each satellite and $t_m = \frac{T_m}{p_m^t} $, $h_m = \frac{H_m}{p_m^h} $, $w_m = \frac{W_m}{p_m^w} $. Subsequently, we project the $c_m$ dimensions into an embedding of fixed dimension $d$, resulting in an image embedding structured as a dictionary with dimensions $[B, t_m, h_m, w_m, d]$ for each modality.

\paragraph{Spatial encoder} We unify the dictionary into a tensor array by padding tensors from different satellites to the same dimensions, yielding $M$ tensors of size $[B, t, h, w, d]$. Here, $t, h,$ and $w$ represent the maximum temporal and spatial dimensions across all satellites. We add spatial encodings to tensors. Subsequently, we concatenate these tensors along the batch dimension, resulting in a shape of $[MB, t, h, w, d]$. We then reshape the tensor into $[MBt, hw, d]$, enabling the spatial encoder to concentrate on processing tokens from spatial dimensions. This approach allows all satellite modalities to share one spatial encoder while preserving the temporal dimension during spatial processing. The padded regions of tensors are disregarded during attention layers, ensuring the spatial encoder can accommodate modalities with varying dimensions effectively. We use the architecture of standard transformer encoder here.

\paragraph{Temporal encoder} Following the spatial dimension processing, our focus shifts to the temporal dimension. We rearrange the tensors into $[MBhw, t, d]$ and concatenate the sequence with $K$ class queries ($[MBhw, t+K, d]$). Subsequently, we add temporal encodings and feed the tensors to a standard transformer encoder. To eliminate the temporal dimensions, we retain only the $K$ embeddings from the class queries ($[MBhw, K, d]$), as introduced in \cite{tarasiou2023TSViT} and then we reshape the tensors into $[MBK, hw, d]$

\paragraph{Multi-modality decoder} In both the spatial and temporal encoders, we treat image embeddings from each satellite modality independently. The multi-modality decoder is crafted to encourage interaction among different modalities. This is achieved by employing the embedding from one satellite modality as queries ($[BK, hw, d]$) and the embeddings from others as keys and values. We utilize embeddings from the modality that shares the same spatial resolution as the reference data as queries. Such an approach compels the standard transformer decoder to extract features from other modalities based on the information provided by one modality. For example, we may choose to query features from Sentinel-1 SAR images based on Sentinel-2 optical images. 

\paragraph{Segmentation head} In the final step, we employ a Multilayer Perceptron (MLP) to project the output of the decoder into $[BK, hw, p^h\times p^w]$ and reshape it into $[B, H, W, K]$, where $H$ and $W$ represent the original spatial dimensions of the satellite modality used for querying.

==> not_used/sec/related_work.tex <==
\section{Related Work}
